Spatio-Temporal Action Graph Networks

Events defined by the interaction of objects in a scene are often of critical importance; yet important events may have insufficient labeled examples to train a conventional deep model to generalize to future object appearance. Activity recognition models that represent object interactions explicitly have the potential to learn in a more efficient manner than those that represent scenes with global descriptors. We propose a novel inter-object graph representation for activity recognition based on a disentangled graph embedding with direct observation of edge appearance. We employ a novel factored embedding of the graph structure, disentangling a representation hierarchy formed over spatial dimensions from that found over temporal variation. We demonstrate the effectiveness of our model on the Charades activity recognition benchmark, as well as a new dataset of driving activities focusing on multi-object interactions with near-collision events. Our model offers significantly improved performance compared to baseline approaches without object-graph representations, or with previous graph-based models.

==> Sections/07_discussions.tex <==
% section{Discussion}
\label{sec:discussion}

Our proposed model architecture mainly addresses the use case where there are prominent objects and their relations in a driving scene which determine the activity class. In future work we would like to address more complex scenarios of activities and scenes which contain high order of complexity between multiple objects. An example for such a use case for activity recognition in the driving field could be understanding third party collisions, which could be useful in a real life scenarios. 


% We already collected a few hundred dash-can videos with third party collisions on which we will test our approach.


% In order to use our object-aware action recognition approach on such cases, there is a need to do a temporal alignment of all the objects in the scene. 

==> Sections/backup_01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Teaser Figure
\begin{figure}[t!]
	\begin{center}
        \includegraphics[width=0.8\linewidth]{Figures/teaser_fig5.jpg}
    \vspace{-10pt}
	\caption{\small{Our  Spatio-Temporal Action Graph (STAG) approach models inter-object relations per frame. Each frame representation contains objects (a) and their relations (b). Our model contains two hierarchies: a spatial hierarchy to model all possible object interactions in a frame and a temporal hierarchy to aggregate the temporal context for the whole video.}}
	\vspace{-25pt}
	\label{fig:tesear}
	\end{center}
\end{figure}


%Streaming image data is becoming more and more prevalent, % tends to burst out as more video 
%as video recording appliances are more embedded in our daily life.
%Dashcam and traffic surveillance videos, in particular, are becoming readily available in large quantity, and automatically classifying events in these videos could greatly save human labor relative to current manual review and reporting systems, and ideally lead to  autonomous driving or alerting systems with fewer accidents, injuries, and deaths overall. 
%\{not sure we need this paragraph, but I polished it anyway.}
%This pose the demands of defining more accurate models for video classification.

%Recognition of complex events in natural scenes poses a challenge for deep learning approaches, since conventional approaches can fail to represent important interactions in a scene, which current models are overlooking of the important cues that are relevant for interpreting the activity in the scene. For example, in driving scenarios critical events are often a function of the spatial relationship of prominent objects, yet those are mostly have been overlooked since it is hard to distinguish their relevance to the event. 




Recognition of events in natural scenes poses a challenge for deep learning approaches to activity recognition, since an insufficient number of training examples are typically available to learn to generalize to all required observation conditions and variations in appearance. For example, in driving scenarios critical events are often a function of the spatial relationship of prominent objects, yet available event training data may not exhibit variation across a sufficiently wide range of appearances.
%
%
%Conventional deep models work well when they are supervised across the range of conditions they will experience, and conversely, may perform poorly on new object-appearance combinations; 
E.g., if a conventional deep model has only seen red pickup trucks rear-end blue sedans, and green trucks always drive safely in the training set, it may perform poorly in a test condition when observing a green pickup truck that is actually about to hit a red sedan.  
It is thus important to develop activity recognition models that can generalize effectively across object appearance and inter-object interactions.  

Early deep learning approaches to activity recognition were limited to scene-level image representations, directly applying convolutional filters to full video frames, and thus not modeling objects or their interactions explicitly \cite{donahue2015long,tran2015learning,simonyan2014two}.
\comment{Typical methods of this type included an LSTM conditioned on per-frame CNN features~\cite{donahue2015long}, 3D ConvNets \cite{tran2015learning} and two-stream ConvNets~\cite{simonyan2014two}. 
}


Although networks are growing deeper and wider, the method for extracting features from network backbones is often still a basic pooling operation, with or without a pixel-wise attention step. These conventional deep learning approaches are unable to directly attend to objects or their spatial relationships explicitly.

A natural approach to the above problem is to build models that can capture relations between objects across time. This object-centric approach can decouple the object detection problem (for which more data is typically available. e.g., images of cars) and the problem of activity recognition. %Here we show how to build such models, and demonstrate their empirical effectiveness in activity recognition. 
Many classic approaches to activity recognition explored object-based representations  \cite{gkioxari2015finding,weinzaepfel2016towards,mettes2017spatial,packer2012combined, brendel2011learning,gupta2009observing}; yet with conventional learning methods such approaches did not show significant improvements in real-world evaluation settings.
Several deep models have been recently introduced that directly represent objects in video in activity recognition tasks. For example \cite{baradel2018object} uses a relation network followed by an RNN, and \cite{wang2018videos} uses a spatio-temporal graph constructed whose nodes are object detections. These models showed that a deep model with a dense graph defined over  scene elements can lead to increased performance, but were limited in that only unary object appearance was considered, with a fully-connected spatio-temporal graph. %Clearly, many such models are possible, and the goal is to design an architecture with that on the one hand provides a detailed representation of inter-object relations with relatively few parameters, while on the other hand performing simple aggregation in time.

% \roeih{Our model is the first to explicitly represent inter-object relations for activity recognition, and do so without explicit supervision on where the objects are, what they are, and how they interact. We achieve this via a \textbf{latent temporal relation} graph model for activity recognition that explores the \textbf{visual interaction} between the objects. Our experiments prove that modeling the visual appearance between objects outperforms other techniques (e.g. similarity and concatenation) for object-object interactions. Moreover, we trained our model to predict activity, as a down-stream task without the full supervision of relations data, which are considered costly to collect.} 

In this paper we propose a novel Spatio-Temporal Action Graph (STAG), which offers improved activity recognition. \roeih{Our model is the first to explicitly represent inter-object relations for activity recognition, and do so without explicit supervision on where the objects are, what they are, and how they interact.} First, we observe that relations between objects are captured in the bounding box containing both objects more effectively than in the object boxes individually. Our graph utilizes explicit appearance terms for edges in the graph, forming a type of ``visual phrase'' term for each edge~\cite{visualphrases}: edge weights in our graph are formed using a descriptor pooled over the spatial extent of the union of boxes of each object pairs. \roeih{Our experiments prove that modeling the visual appearance between objects outperforms other techniques (e.g. similarity and concatenation) for object-object interactions.}

Second, we propose a disentangled spatio-temporal embedding of our graph, factoring spatial and temporal connections into two hierarchies which refine the edges considering all possible relations in a frame jointly over space, or over time, but not both. In our spatial hierarchy relations are refined by considering all possible relations in a frame jointly. We therefore obtain relation descriptors for each possible object-pair in each frame. Then, we use attention across relations to generate one relation descriptor per frame. This can be thought of as the salient relation in the current frame. Next, we use the temporal hierarchy to aggregate the temporal context for the whole video. We perform attention across all frames to extract one descriptor for the entire video, which is used as input to the classifier. We argue that this architecture is ideally structured for capturing relations that underlie typical actions in video. Indeed our empirical results show that it outperforms other spatio-temporal approaches, including LSTM based ones.

\roeih{
Another key contribution of our work is a new dataset\footnote{Upon acceptance of our paper, we will make a public release and challenge based on this dataset.} for activity detection in driving. Activity recognition is of key importance in the domain of autonomous driving, in particular detecting collisions or near-collisions is of utmost importance. Most of the research on this topic is in simulation mode, and we introduce the first attempt to studying it in real world data. Additionally, this is the first dataset containing object-object interactions, while the current activity recognition datasets are human-object interactions that have small number of objects per scene. Thus, they cannot contain rich relation information. Here we provide a new dataset which will allow researchers to study recognition of such rare and complex events. Our Collision dataset was collected from real-world dashcam data consisting of 803 videos containing collisions or near-collisions from more than ten million rides.\footnote{There are only relatively few collision videos, since naturally, such events are rare.} In \figref{fig:tesear}, we demonstrate our approach on a driving scene for collision event detection.}


% Another key contribution of our work is a new dataset for activity detection in driving. Activity recognition is of key importance in the domain of autonomous driving. In particular detecting collisions or near-collisions is of utmost importance. Here we provide a new dataset which will allow researchers to study recognition of such rare and complex events. Our Collision dataset was collected from real-world dashcam data consisting of 803 videos containing collisions or near-collisions from more than ten million rides.\footnote{There are only relatively few collision videos, since naturally, such events are rare.} \roeih{In addition, most of the research on this topic is in simulation mode, and we introduce the first attempt to studying it in real world data (we are not aware of any other real-life collision dataset until our submission). Additionally, this is the first dataset containing object-object interactions, while the current activity recognition datasets are human-object interactions that have small number of objects per scene. Thus, they cannot contain rich relation information.} In \figref{fig:tesear}, we demonstrate our approach on a driving scene for collision event detection.\footnote{Upon acceptance of our paper, we will make a public release and challenge based on this dataset.}

% \roeih{Our dataset has been collected from $10^6$ rides of real life driving dash cams. Collisions are an extremely rare event since they appear in less than 1\% of driving time, and therefore collecting them is a challenging problem. To our knowledge, this is the first dataset containing such rare and important data, and therefore it has great potential and significance for the vision community, and in particular for research on autonomous vehicles. In addition, most of the research on this topic is in simulation mode, and we introduce the first attempt to studying it in real world data. Additionally, this is the first dataset containing object-object interactions with an average of more than $6$ different objects in a scene, while the current activity recognition datasets are human-object interactions that have $3$ objects per scene at most. Thus, they cannot contain rich relation information.}


We evaluate our STAG model on both the Collision dataset as well the Charades~\cite{sigurdsson2016hollywood} activity recognition benchmark, demonstrating improvement over previous baselines. Our results confirm that the use of explicit object representations in spatial-temporal hierarchy can offer better generalization performance for deep activity recognition in realistic conditions with limited training data.






==> Sections/backup_05_experiments_charades.tex <==
\section{Experiments on the Collision Dataset}
\label{sec:exper}
We next describe the results of applying our STAG model to the Collision dataset introduced in~\secref{sec:dataset}. We study model variants and compare it to the state of the art activity recognition models. 




\subsection{Implementation Details}
\label{sec:exper:details}

%%% Model Details %%%
\noindent \textbf{Model Details.} % \quad
We use Faster R-CNN with ResNet50 as a backbone, taking a sequence of $T=20$ frames, and generating bounding box proposals for each of the $T$ frames. Specifically, the strides in FPN are set as the same as \cite{fpn}.
% Specifically, the strides in FPN are set as {(4, 8, 16, 32, 64)}, and for the RPN we set the anchor scales as {(32, 64, 128, 256, 512)}, aspect ratios as {(0.5, 1, 2)} and anchor stride as $1$.  

The input frames are resized to the maximum dimension of 256 with padding. Considering the training time and memory limit, we take the top $N=12$ region proposals on each frame after non-maximum suppression with IoU threshold 0.7, which are sufficient for capturing the semantic information on the Collision dataset. Features for the $N=12$ objects and $N\cdot N$ object interaction relations are extracted following~\secref{sec:model}, resulting in feature representations $\zz_i$ for objects and $\zz_{i,j}$ for relations.
% To make Faster R-CNN more adaptive to driving scene, we pretrained it on the BDD dataset~\cite{Madhavan_bdd} using the default data split as the author suggests.

%%% Training Details %%%
% \noindent \textbf{Training Details.} % \quad
\noindent \textbf{Training and Inference.} % \quad
We train the STAG model using SGD with momentum $0.9$ and an initial learning rate $0.01$. The learning rate was decayed by a factor of $0.5$ each epoch, and the gradient was clipped at norm $5$. Each batch includes a video segment of $T$ frames.
Two kinds of ground truth data are utilized during training, namely the ground truth bounding box annotations on each frame and the collision label per segment. 
% The detection annotations came from the pretrained Faster-RCNN, which is pretrained on BDD~\cite{Madhavan_bdd}.
% The loss of our STAG model for Object-Aware Activity Recognition contains two components: the bounding box localization related losses used in the Faster-RCNN detector of the STAG model and the multi-class activity classification loss. The Faster-RCNN detector is trained with RPN classification and regression losses, and the classification and regression in the second stage, as is standard with two stage detectors. The two losses used in the two stages are given equal loss weights. To train our STAG model for collision prediction, we apply a binary cross entropy loss between the binary collision prediction logit and the ground-truth collision label. 

The loss of our STAG model for Object-Aware Activity Recognition contains two components: the bounding box localization related losses used in the Faster-RCNN detector of the STAG model and the multi-class activity classification loss, as is standard with two stage detectors. To train our STAG model for collision prediction, we apply a binary cross entropy loss between the binary collision prediction logit and the ground-truth collision label. 



\comment{
% Model details
\subsection{Model Details}
\label{sec:exper:details}

We use Faster R-CNN with ResNet50 as a backbone, taking a sequence of $T=20$ frames, and generating bounding box proposals for each of the $T$ frames. Specifically, the strides in FPN are set as {(4, 8, 16, 32, 64)}, and for the RPN we set the anchor scales as {(32, 64, 128, 256, 512)}, aspect ratios as {(0.5, 1, 2)} and anchor stride as $1$. 
The input frames are resized to the maximum dimension of 256 with padding.
Considering the training time and memory limit, we take the top $N=12$ region proposals on each frame after non-maximum suppression with IoU threshold 0.7, which are sufficient for capturing the semantic information on the Collision dataset.
%Using a higher number or ROIs could potentially be a major issue for time and space complexity. However, meaningful scene could be represented by only 12 objects because they capture sufficient information of the scene.
%We are training with a ratio of 1 to 3 between positive and negatives\amirg{What's positive and negative here? If it's the classes then it should not be in this part.}. 

Features for the $N=12$ objects and $N\cdot N$ object interaction relations are extracted following~\secref{sec:model}, resulting in feature representations $\zz_i$ for objects and $\zz_{i,j}$ for relations.
To make Faster R-CNN more adaptive to driving scene, we pretrained it on the BDD dataset~\cite{Madhavan_bdd} using the default data split as the author suggests.



% Training Section
\subsection{Training Details}
\label{sec:exper:train}
We train the STAG model using SGD with momentum $0.9$ and an initial learning rate $0.01$. The learning rate was decayed by a factor of $0.5$ each epoch, and the gradient was clipped at norm $5$. Each batch includes a video segment of $T$ frames.
Two kinds of ground truth data are utilized during training, namely the ground truth bounding box annotations on each frame and the collision label per segment.
The detection annotations came from the pretrained Faster-RCNN, which is pretrained on BDD~\cite{Madhavan_bdd}.
The loss of our STAG model for Object-Aware Activity Recognition contains two components: the bounding box localization related losses used in the Faster-RCNN detector of the STAG model and the binary/multi-class activity classification loss.\ag{Is it binary or multi-class? How many categories?} 
The Faster-RCNN detector is trained with RPN classification and regression losses, and the classification and regression in the second stage, as is standard with two stage detectors. The two losses used in the two stages are given equal loss weights. 
To train our STAG model for collision prediction, we apply a binary cross entropy loss between the binary collision prediction logit and the ground-truth collision label. 

% Training: Spatio-Temporal Action Graph Network
%\textbf{Spatio-Temporal Action Graph Classification Loss}
%The Spatio-Temporal Action Graph network (\secref{sec:model:actions_net}) has two logits at its output, 
%corresponding to the two possible actions ("collision" or "no collision"). Since we have the ground-truth for this class, 



%We trained the Object-aware Activity Recognition with a ratio of 1:3 of positive to negatives, meaning the Spatio-Temporal Action Graph was able to learn both positive and negatives examples.
%  The loss of the Object-aware Activity Recognition was a sum of the following two components: the Mask-RCNN detector and the Spatio-Temporal Action Graph network. We trained the 
% Object-aware Activity Recognition with a ratio of 1:3 of positive to negatives.
% Training: Detector
%\textbf{Detector}. The Backbone and RPN are trained in with a loss that consisting of RPN classification and regression, and the classification and regression of the second stage, as is standard with two stage detectors. The two losses are given the same weight. 

% Training: Spatio-Temporal Action Graph Network
%\textbf{Spatio-Temporal Action Graph Classification Loss}
%The Spatio-Temporal Action Graph network (\secref{sec:model:actions_net}) has two logits at its output, corresponding to the two possible actions ("collision" or "no collision"). Since we have the ground-truth for this class, we simply use a binary cross entropy loss between the logits and the ground-truth label. 
}

% Charades Space figure
\begin{figure*}[t!]
    \begin{center}
        \includegraphics[width=0.7\linewidth]{Figures/demo_space.pdf}
    \caption{hehe}
    \label{fig:charades_space}
    \end{center}
    % \vspace{-10pt} 
\end{figure*}

% Model Ablations section
\subsection{Model Variants}
\label{sec:exper:ablations}
We refer to our full model as a \texttt{Spatio-Temporal Action Graph} (\texttt{STAG}). STAG progressively processes the box features and the spatial appearance features of pairwise boxes $\zz_i^t,\zz_{i,j}^t$ into a single vector for final activity recognition, with hierarchical structure encoding. To show the superiority of our STAG model with two specific spatial and temporal attention hierarchies, we design two model variants for comparison.
\newline
(1) \texttt{LSTM Spatial Graph} - We study the effect of the STAG ``Temporal Context Hierarchy'' stage, as  compared to a recurrent neural network based solution. To do so, we replace the ``Temporal Context Hierarchy'' stage with an LSTM that processes the same tensor of size $T\times d$.
%at time $t$ is the $\ve'{_{i}^{t}}$ vector in \figref{fig:actions_graph} 
%this model replaces the final attention-based reduction step in STAG with LSTM reduction.
%(i.e., the output of $\gamma$ function). Thus,
(2) \texttt{LSTM Boxes} - We study the effectiveness of effect of representing object interactions. To do so, we replace the  STAG ``Spatial Context Hierarchy'' stage with just average pooling of the individual node features, to obtain a tensor of size $T\times d$.
%To show the usefulness of the spatial encoding in original STAG with spatial appearance of pair-wise box features, on top of \texttt{LSTM Spatial Graph}, we further replace the spatial encoding to be simply pooling of object node features without bounding box spatial layout consideration.
%\roeih{If the purpose is to show what you claimed then why using LSTM? you refer this part in the ablation section. Therefore, I propose to remove 1 and put the explanation of 1 here}

%An LSTM model whose input at time $t$ are the RPN features for the $B$ boxes. This model does not use any component in \figref{fig:actions_graph}. The final state of the LSTM is used for predicting the binary action label ``collision'' or ``no collision''. \\ 

%Another approach to capturing temporal structure are recursive neural nets and in particular LSTM. 
%Here we describe two LSTM variants that use some aspects of STAG, but replace the temporal processing in STAG with an LSTM model. 
%get in each frame the boxes and after sequence of $T$ frames outputs a prediction.
We also train two other popular activity recognition models on Collision dataset: the C3D model~\cite{tran2015learning} and I3D model~\cite{Carreira2017QuoVA}.
We used pretrained weights for C3D and I3D. The C3D was pretrained on Sports-1M while the I3D was pretrained on imagenet.


% We finetune the Sports-1M pretrained C3D weights on the Collision dataset. I3D model with kinetics data pretrained.


%which 
%at each frame the input is a graph feature representation, and predicts after sequence of $T$ frames "collision" or "no collision". \\

% (4) \textsc{Baseline-Model}.
%Comparing the \textsc{LSTM BOXES} to \textsc{LSTM SPATIAL GRAPH}/ \textsc{SPATIO-TEMPORAL ACTION GRAPH} allows to evaluate the benefit of learning a scene representation and explore whether the Action Graph Network is beneficial for activity recognition.

%Comparing the \textsc{SPATIO-TEMPORAL ACTION GRAPH} / \textsc{LSTM SPATIAL GRAPH} to \textsc{C3D} allows to evaluate the benefit of graph networks vs 3D convolutions vs RNN/LSTM. 

% Baseline
%\subsection{A C3D Baseline}
%\label{sec:exper:baseline}
%\roeih{Huijuan, please fill this section on C3D. its our baseline.}
%We compare our approach with the C3D \cite{tran2015learning} approach, which uses a 3D ConvNet to extract rich spatio-temporal feature hierarchies from a given input video buffer.
%We adopt the convolutional layers (\texttt{conv1a} to \texttt{conv5b}) and fc layers(\texttt{fc6} to \texttt{fc8}) of C3D model\ag{Not clear what this means}.
%The input to our model\ag{Do you mean our model, or the C3D baseline?} is a sequence of RGB video frames with dimension $\mathbb{R}^{3\times L\times H\times W}$.
%The height ($H$) and width ($W$) of the frames are taken as 112 each following~\cite{tran2015learning}.
%The number of frames $L$ is set as 16 frames sampled from each video\ag{Why is this not 20 like in STAG?}.
%We use the Sports-1M pretrained C3D weights to initialize the model.


%In order to show the complementary effect of the video feature encoding using spatio-temporal filters, we fuse the prediction from the C3D model and our proposed STAG model by averaging the classification scores from both models.
%Similarly, the C3D model is fused with other model variants \texttt{LSTM Boxes} and \texttt{LSTM Spatial Graph} (listed in \secref{sec:exper:ablations}).

%Finally, we also consider a simple fusion of C3D and STAG, where the output logits are averaged. Similarly, C3D is fused with the variants in \secref{sec:exper:ablations}.
%the late fusion showed us that 3D are also helpful when combining the two together
%\huijuan{need to add one or two sentences about fusion}


% % Comparing Blocks figure
% \begin{figure}[t!]
%     \begin{center}
%         \includegraphics[width=0.8\linewidth]{Figures/comparing_blocks_iccv.jpg}
%     \caption{Comparison between three different dimension reduction methods for feature aggregation. (a) Standard pooling over the spatial dimension. (b) A standard Non-Local (NL) block \cite{Wang_videogcnECCV2018} to get improved features and then pooling. (c) Our proposed \textbf{Context Hierarchy Block}: combining the residue of pooling and original features to our proposed Hierarchy Non-Local block. \roeih{we are comparing later between (b) and (c)}}
%     \label{fig:comparing_blocks}
%     \end{center}
% \end{figure}

% Results




\subsection{Results}
We first compare the STAG results on the full dataset to the model variants described in \secref{sec:exper:ablations}. ~\tabref{sec:exper:results} reports classification accuracy. Firstly, STAG outperforms all the other models including C3D and I3D. Replacing the temporal processing in STAG with an LSTM as in \textsc{LSTM Spatial Graph}, we get 7\% accuracy decrease, showing the superiority of our temporal modeling over LSTM. Further removing the pairwise object modeling, we see accuracy further decrease by 8\% in \textsc{LSTM Boxes}. 

Finally, we consider a simple ensemble model of STAG and C3D by simply averaging their output scores. Results of this combination are shown in Table \ref{sec:exper:fusion_results}. We can see the combination improves the original C3D accuracy, showing the benefits of object interaction modeling. Among all the ensemble results, the STAG model still maintains the highest accuracy result 85.5\%.

We also show the results on the few-Shot dataset in \tabref{sec:exper:results} and \tabref{sec:exper:fusion_results}. It can be seen that the two model variants \textsc{LSTM Spatial Graph} and \textsc{LSTM Boxes} almost fail on this challenging few-shot dataset. Although our STAG model achieves marginal improvement compared to the C3D and I3D, the relative low accuracy numbers highlight the challenges of this few-shot Collision dataset.\footnote{We note however, that all these models are not specifically designed for the few-shot setting.} We encourage the whole community to further develop few-shot based activity recognition models to tackle this challenging few-shot dataset.


\comment{
To see the complementary strengths of STAG with hierarchical object interaction modeling to C3D, we fuse the prediction from C3D with STAG model and its variants \textsc{LSTM Spatial Graph} and \textsc{LSTM Boxes}.}


% We also show the results on the few-Shot dataset in \tabref{sec:exper:results} and \tabref{sec:exper:fusion_results}.
% It can be seen that the two model variants \textsc{LSTM Spatial Graph} and \textsc{LSTM Boxes} with accuracy around 67\% almost fail on this challenging few-shot dataset. Although our STAG model (73.8\%) achieves marginal improvement compared to the C3D (72\%) and I3D (73.6\%), the relative low accuracy numbers highlight the challenges of this few-shot Collision dataset.\footnote{We note however, that all these models are not specifically designed for the few-shot setting.} We encourage the whole community to further develop few-shot based activity recognition models to tackle this challenging few-shot dataset.

\subsection{Ablation Studies}
We also design some direct ablation studies for the components in our STAG model. We refer to our edges descriptors processing as \texttt{Node Interactions} in ~\tabref{sec:exper:results}. To validate the effectiveness of our disentangled spatio-temporal hierarchies, we design two ablation studies for the two attention hierarchies: 
(1) \texttt{STAG Space} - Replacing the spatial hierarchy by directly pooling.
(2) \texttt{STAG Time} - Replacing the temporal hierarchy by directly pooling.

The results are shown in Table~\ref{sec:exper:hier_ablations}. From the results, we can see that both ablations decrease accuracy, but that the temporal hierarchy has a larger effect on performance.

Furthermore, we explore the use of different edge features in Table~\ref{sec:exper:hier_ablations}: 
(1) \texttt{STAG Cat} - Set the edge feature to be just the concatenation the corresponding node features (i.e., union box is not used).
(2) \texttt{STAG Sim} - Set the edge features to be the multiplication of the two corresponding node features, as in \cite{Wang_videogcnECCV2018}.

Both methods result in approximately two point accuracy decrease, indicating the superiority of using spatial appearance features of union boxes as edge features in our hierarchical STAG models.


\ignore{
\subsubsection{Qualitative Analysis}
\huijuan{consider removing this section, since this just visualize video frames and predicted labels without attention weights...}
Visual inspection of success and failure cases reveals an interesting pattern. We observe that STAG outperforms C3D on ``near-collision'' cases such as that in the upper row of \figref{fig:exper:full}. Correctly classifying such cases requires understanding the relative configuration of the objects in order to determine if there was an incident or not. On the other hand C3D may put too much weight on events such as speed-change which are not always predictive of an accident.
The C3D model outperforms STAG on cases where objects are not clearly visible. For example in the lower row of  \figref{fig:exper:full}.
}


%%%%%%%%%%%%%%%%%%%%%%%
% Results Full figure %
%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/results_analysis2.jpg}
\caption{Success and failure cases for STAG. {\bf Top Row}: a near-collision example (i.e., the correct label is ``no collision'') 
where the STAG model correctly classifiers, and the C3D model does not. {\bf Middle Row}: a collision example (i.e., the correct label is ``collision''), where the C3D model is correct, while the STAG module errs. {\bf Bottom Row}: a collision example (i.e., the correct label is ``collision''), where the STAG module which was trained on the Few-shot dataset is correct.}
\label{fig:exper:full}
\end{center}
\end{figure*}
}


%%%%%%%%%%%%%%%%%%
% Models Results%%
%%%%%%%%%%%%%%%%%%

\begin{table}[t!]
\begin{center}

\label{results}
\small
   \begin{tabular}{|l|cc|} 
     \hline
     \multicolumn{1}{|c|}{} &    \multicolumn{2}{c|}{Accuracy} \\
    %  \multicolumn{1}{|c|}{Full Dataset} &
    %  \multicolumn{1}{c|}{Few-shot Dataset}\\
     {} & {Full Dataset} & {Few-shot Dataset} \\
     \hline
     I3D & 82.4 & 73.6 \\ 
     C3D & 79.9 & 72 \\ 
     LSTM Spatial Graph & 77.5 & 67 \\
     LSTM boxes & 69.5 & 69 \\
    % \midrule
     \hline
     \textsc{STAG} & \textbf{84.5} & \textbf{73.8} \\
     \hline
\end{tabular}
  %\vspace{-10pt}
  \caption{Classification accuracy on the Collisions dataset for the STAG model and its variants, and the C3D \& I3D model.}
  \label{sec:exper:results}
\hspace{2.0cm}
\end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%
% Fusion Models Results%
%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t!]
\begin{center}
\label{results}
\small
  \begin{tabular}{|l|cc|}
     \hline
     \multicolumn{1}{|c|}{} &
     \multicolumn{2}{c|}{Accuracy} \\
     {} & {Full Dataset} & {Few-shot Dataset} \\
     \hline%\hline
     LSTM spatial Graph & 83.56 & 73.1 \\
     LSTM boxes & 81.2 & 72.3 \\
     %\midrule
     \hline
     \textsc{STAG} & \textbf{85.5} & \textbf{74.4} \\
     \hline
\end{tabular}
  %\vspace{-10pt}
  \caption{Classification accuracy on the Collisions dataset for STAG model and variants, when averaged with the C3D model.}
  \label{sec:exper:fusion_results}
\hspace{2.0cm}
\end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%
% Hierarchy Ablations   %
%%%%%%%%%%%%%%%%%%%%%%%%%

%---------------------------
% Hierarchy Charades Table
%---------------------------

\begin{table}[t] 
    \small
    \centering
    % \resizebox{\linewidth}{!}
    {
    \begin{tabular}{lllc}
        & \textbf{Edge} & \textbf{Hierarchy} & \textbf{Accuracy} \\
        \toprule
        STAG Cat & Node concat. & - & 83.1 \\
        STAG Sim & Cosine sim. & - & 83.5 \\
        \midrule
        STAG Time & Node interactions & Time only & 78.8 \\
        STAG Space & Node interactions & Space only & 82.6 \\
        \textbf{STAG Full} & Node interactions & Space \& Time & \textbf{84.5} \\
        \bottomrule
        \addlinespace
    \end{tabular}
    }
    \vspace{-14pt}
    \caption{Hierarchy \& Edge features Ablations on the Collision dataset.}
    %\vspace{-14pt}
    \label{sec:exper:hier_ablations}
\end{table}



% \begin{table}[t]
%     \small
%     \centering
%     % \resizebox{\linewidth}{!}
%     {%
%     \begin{tabular}{llc}
%         & \textbf{Hierarchy}
%         & \textbf{Accuracy}
%         \\
%         \toprule
%         STAG Space & space only & 82.6 \\
%         STAG Time & time only & 78.8 \\
%         STAG & space \& time & 84.5 \\
%         \bottomrule
%         & \textbf{Edge} & \textbf{Accuracy} \\
%         \toprule
%         STAG Cat & Node concat. & 83.1 \\
%         STAG Sim & Cosine sim.~\cite{Wang_videogcnECCV2018} & 83.5 \\
%         STAG & Node interactions & \textbf{84.5} \\
%         \bottomrule
%         \addlinespace
%     \end{tabular}
%     }
%     \vspace{-14pt}
%     \caption{Hierarchy \& Edge features Ablations on the Collision dataset.}
%     %\vspace{-18pt}
%     \label{sec:exper:hier_ablations}
% \end{table}

% \begin{table}[t!]
% \begin{center}
% \label{results}
% \small
%   \begin{tabular}{|l|c|} 
%      \hline
%      \multicolumn{1}{|c|}{}&\\
%     %  \multicolumn{2}{c|}{Accuracy} \\
%      {Hierarchy Ablations} & {Accuracy}\\
%      \hline%\hline
%      \texttt{No Hierarchy 1} & ? \\
%      \texttt{No Hierarchy 2} & ? \\
%      %\midrule
%      \hline
%      \textsc{Full Hierarchy} & \textbf{84.5} \\
%      \hline
% \end{tabular}
%   \caption{Hierarchy Ablations on Collision Dataset.}
%   \label{sec:exper:hier_ablations}
% \hspace{2.0cm}
% \end{center}
% \end{table}


% % Interoperability and Explainability figure
% \begin{figure*}[t!]
%     \begin{center}
%         \includegraphics[width=\linewidth]{Figures/interoperability_explainbility2.jpg}
%     \caption{{\bf Explainability via Attention}. A sequence of frames, with superimposed heat-map as calculated using the attention component in \figref{fig:actions_graph}. It can be seen that more ``dangerous'' objects tend to receive more attention.}
%     \label{fig:attention_graph}
%     \end{center}
% \end{figure*}


% Charades Time figure
\begin{figure*}[t!]
    \begin{center}
        \includegraphics[width=\linewidth]{Figures/demo_time.pdf}
    \caption{}
    \label{fig:charades_time}
    \end{center}
\end{figure*}

% \begin{figure*}
%   \subfloat{\label{fig:attention_graph}\includegraphics[width=\linewidth]{Figures/interoperability_explainbility2.jpg}}
%   \subfloat{\label{fig:2}\includegraphics[width=\linewidth]{Figures/demo_time.pdf}}
%   \caption{Caption of both figures}
%   \label{fig:pics}
% \end{figure*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge Collision Ablations   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t] 
%     \small
%     \centering
%     % \resizebox{\linewidth}{!}
%     {
%     \begin{tabular}{llc}
%         & \textbf{Edge} & \textbf{Accuracy} \\
%         \toprule
%         STAG Cat & Node concat. & 83.1 \\
%         STAG Sim & Cosine sim.~\cite{Wang_videogcnECCV2018} & 83.5 \\
%         STAG & Node interactions & \textbf{84.5} \\
%         \bottomrule
%         \addlinespace
%     \end{tabular}
%     }
%     %\vspace{-14pt}
%     \caption{Edge features ablations on the Collision dataset.}
%     %\vspace{-14pt}
%     \label{sec:exper:edge_ablations}
% \end{table}


% \begin{table}[t!]
% \begin{center}
% \label{results}
% \small
%   \begin{tabular}{|l|c|} 
%      \hline
%      \multicolumn{1}{|c|}{}&\\
%     %  \multicolumn{2}{c|}{Accuracy} \\
%      {} & {Accuracy}\\
%      \hline%\hline
%      \texttt{Boxes concatenation} & 83.1 \\
%      \texttt{Boxes multiplication} & 83.5 \\
%     %  \texttt{Boxes concatenation} & 81.69 \\
%     %  \texttt{Boxes multiplication} & 80.28 \\
%      %\midrule
%      \hline
%      \textsc{Union Boxes} & \textbf{84.5} \\
%      \hline
% \end{tabular}
% \vspace{-10pt}
%   \caption{Edge features ablations on Collision Dataset.}
%   \label{sec:exper:hier_ablations}
% \hspace{2.0cm}
% \end{center}
% \end{table}
     
     
% What the model learns
\ignore{
\subsection{Attention Visualization}
\huijuan{please double check....}
\ag{We no longer call it attention in the STAG explanation, so either say there that NLM is essentially attention or do the switch here.}
Our STAG model uses attention across space and time to reduce a video into a single vector. One advantage of attention models is their interpretability. Specifically, one can view the attention map in the STAG model to understand which parts of the input have more influence on the decision. 
%For the case of collision detection, this is clearly an important feature.
%One of the main implication of our STAG model is the ability to show what the model learned and hopefully it could be useful to understand how the model works. 
\figref{fig:attention_graph} provides a nice illustration of the insight that attention maps provide. The figure shows heat maps per scene for the attention maps used in the spatial hierarchy. 
The temporal attention connection is shown in the series of bounding boxes.
It can be seen that objects that pose more danger to the driver tend to receive higher
attention values.

%we could see the interpretation of model, while it training to predict collision. Per scene (frame), each object has different confidences (using our attention mechanism, as described in~\secref{sec:model}.), such it able to understand exactly what are the main objects in scene and their level of danger. 
}




















%%%%%%% FROM HERE %%%%%%%




\section{Experiments on the Charades Dataset}
To further validate the effectiveness of our model on publicly available action recognition benchmarks, we also evaluate it on Charades dataset~\cite{sigurdsson2016hollywood}.
We follow the official split (8K training and 1.8K validation videos) to train and test our model.
The average video duration is around 30 seconds. 
There are 157 action classes and multiple actions can happen at the same time.
Thus it is essentially a multi-label recognition task without localization on which we report our results by the metric of mean Average Precision (mAP).

\subsection{Implementation Details}
Closely following to the experiment setup as described in STRG~\cite{Wang_videogcnECCV2018}, we first extract detection proposals using the Region Proposal Network (RPN) in \cite{Detectron2018}. Our RPN is a model with ResNet-50 and FPN backbone. It was first pretrained on \hangg{okay, just leave it here and go back later and figure out how many portion we wanna talk about it in the paper and the supp.}

\noindent \textbf{Model Design} \quad
We choose our backbone network as ResNet-50 Inflated 3D ConvNet (I3D) \hangg{decide how do we either refer to papers (xiaolong's page 6) or put it into our supp.} for all of our experiments. 
\hangg{RPNs, RoIAligns, Concats, Archs...}

\noindent \textbf{Training and Inference} \quad 
Our network takes 32 video frames as inputs which are sampled by the frame rate 6fps, making the our input duration up to around 5 seconds. We use the input frames with the spatial resolution as 224~$\times$~224. Following \cite{simonyan2014very}, we apply the same data augmentation by random crops followed by random scales so that the shorter side of the video layout is sampled within [256, 320]. 
For each frame of the inputs, we select top-15 object proposals as the input for the graph nodes.

To train our model, we follow the same training schedule as specified in STRG using a mini-batch of 8 videos for each iteration and repeat it with 100K iterations in total. We apply SGD optimization algorithm with the learning rate of 0.00125 in the first 90K iterations and anneal by 10 during the last 10K iterations. We apply dropout before the final global pooling layer to avoid over-fitting. The training objective for experiments on this dataset is a simple multi-class binary cross entropy loss. 

During inference, we apply multi-crop testing~\cite{wang2018non,Wang_videogcnECCV2018} for better performance. Specifically, we sample 3 crops of size 224~$\times$~224 and 10 clips from each video and rescale the shorter side of each video frame to 256 while maintaining the aspect ratios. The final recognition results are based on late fusion of classification scores.

\subsection{Quantitative Evaluation}
We now quantitatively evaluate our STAG model against public available state-of-the-art approaches on the benchmark. We also ablate over our own design choices to see whether using (1) node interaction as the edge and (2) separate space-time hierarchies help action recognition in general -- and if help, what dynamics between our design components we should expect so as to understand our model better.

\noindent \textbf{Main results} \quad
Table \ref{tab:cha} shows that our STAG model compares favorably against prior works using same ResNet-50 I3D model \hangg{remove nl, more texts.}
% as backbone and comparable against recent Non-local networks \cite{wang2018non} which has roughly 3$\times$ numbers of parameters than ours. 

Building on a simple I3D model, we have achieved 5.4\% absolute performance gain. Compare to our closest previous work STRG which adopts the same backbone, we show 1.0\% performance improvement without applying any tricks. 

\noindent \textbf{Ablations} \quad
We next move on to controlled studies to better understand our design choices. Generally, we control two design factors -- (1) the edge feature and (2) the space-time feature aggregation (hierarchy) -- in our model and recast previous STRG model into this framework for the direct comparison.

As shown in Table \ref{tab:cha_abl}, STRG can be seen as the graph model which uses cosine similarity between the objects nodes as the edge feature, while either not discriminating nodes from different frames at all (STRG Sim) or only applying heuristic backward-forward node association as space-time hierarchy.

First, to understand whether edge feature helps, we have proposed two baselines -- STAG Cat. and STAG Interact. -- which also have no hierarchy for late feature-fusion. By comparing against STRG Sim., it is shown that simply concatenating node feature does not make good edge representation. On the contrary, our design of union box edge feature potentially captures object interactions and bring 0.6\% performance gain over STRG Sim. model. 

Then, to make sense of our hierarchy designs in gap to our full model, we here show another two baseline built on STAG Interact. by removing either space or time hierarchy at a time. It is interesting to see that removing temporal hierarchy will even harm the performance comparing to direct modeling node interaction without discriminating space or time which are used in STAG Interact. We hypothesis that focus on space hierarchy alone is ineffective in the sense that the temporal pooling alone is not enough for feature aggregation. On the other hand, STAG Time model, shows that on Charades 

Results using a ResNet-50 inflated backbone are shown in Table~\ref{tofill}.
we got an improved results using the same ResNet-50 backbone and the ablation studies on two hierarchies show the important role of each hierarchy.\ag{Sentence needs rewriting.} \hangg{this is the old para, to be removed.} 

%dataset introduction
%multi-lables
%evaluation metrics
%R50 backbone.
%Fater RCNN to extract boxes.
%backbone model based on the ResNet-50 architecture, which are
%We take ResNet-50 backbone and inflate it into 3D ConvNet.
%Inflated 3D ConvNet (I3D) [48,8,58] as one can turn a 2D ConvNet into a 3D ConvNet by inflating the kernels during initialization. 
%Region Proposal Network. We apply the 
%Region Proposal Network (RPN) in [79,82] to generate the object bounding boxes of interest on each video frame.
%More specifically, we use the RPN with ResNet-50 backbone and FPN [83].
%The RPN is pre-trained with the MSCOCO object detection dataset [84] and there is no weight sharing between the RPN and our I3D video backbone model. 


%---------------------------
% Results Charades Table
%---------------------------

\begin{table}[t] 
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lllc}
        & \textbf{Backbone} & \textbf{Modality} & \textbf{mAP}
        \\
        \toprule
        2-Steam~\cite{simonyan2014two} & VGG-16 & RGB w/ Flow & 18.6
        \\
        2-Steam w/ LSTM~\cite{simonyan2014two} & VGG-16 & RGB w/ Flow & 18.6
        \\
        Async-TF~\cite{sigurdsson2017asynchronous} & VGG-16 & RGB w/ Flow & 22.4
        \\
        a Multiscale TRN~\cite{zhou2018temporal} & Inception & RGB & 32.9
        \\
        I3D \cite{Carreira2017QuoVA} & Inception & RGB & 32.9
        % \\
        % I3D \cite{wang2018non} & R101-I3D & RGB & 35.5
        % \\
        % I3D-NL \cite{wang2018non} & R101-I3D-NL & RGB & 37.5 
        \\
        \midrule
        I3D \cite{Wang_videogcnECCV2018} & R50-I3D & RGB & 31.8
        \\
        STRG \cite{Wang_videogcnECCV2018} & R50-I3D & RGB & 36.2
        \\
        \textbf{STAG (ours)} \cite{wang2018non} & R50-I3D & RGB & \textbf{37.2}
        \\
        \bottomrule
        \addlinespace
    \end{tabular}
    }
    %\vspace{-14pt}
    \caption{
    \textbf{Cha. \hangg{i just cite the i3d-nl results using r101 backbone -- it's better than use but using a better bb, what should we do about it?}}
    }
    %\vspace{-14pt}
    \label{tab:cha}
\end{table}


%---------------------------
% Edge Ablations Charades Table
%---------------------------

\begin{table}[t] 
    \small
    \centering
    % \resizebox{\linewidth}{!}
    {
    \begin{tabular}{lllc}
        & \textbf{Edge} & \textbf{Hierarchy} & \textbf{mAP} \\
        \toprule
        I3D & - & - & 31.8 \\
        \midrule
        STRG Sim~\cite{Wang_videogcnECCV2018} & Cosine sim. & - & 35.0 \\
        STRG Full \cite{Wang_videogcnECCV2018} & Cosine sim. & Space-time heur. & 36.2 \\
        \midrule
        STAG Cat. & Node concat. & - & 34.5 \\
        STAG Interact. & Node interactions & - & 35.6 \\
        \midrule
        STAG Space & Node interactions & Space only & 34.7 \\
        STAG Time & Node interactions & Time only & 36.6 \\
        \textbf{STAG Full} & Node interactions & Space \& Time & \textbf{37.2} \\
        \bottomrule
        \addlinespace
    \end{tabular}
    }
    %\vspace{-14pt}
    \caption{\hangg{No hier (direct NL and then avg. pool). to compare edge}}
    %\vspace{-14pt}
    \label{tab:cha_abl}
\end{table}

==> Sections/old_02_related_work.tex <==
\section{Related Work}
\label{sec:related_work}


% System Figure
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=\linewidth]{Figures/general_arch_iccv.jpg} % Figures/figure1_arch3.png
\caption{\textbf{Object-aware Activity Recognition architecture}. The input consists of a sequence of 20 frames. (1) A backbone of ResNet50 and RPN produces a set of bounding boxes proposals for each frame. (2) A \textit{RoiAlign Single} layer extracts $\ve_{i}^{t}$ features from the backbone using the boxes. In parallel, every pair of box proposals is used for computing a union box, and  pairwise features $\ve_{i,j}^{t}$ extracted similar to the $\ve_{i}^{t}$ features. (3) The $\ve_{i}^{t}$ and $\ve_{i,j}^{t}$ are used as inputs to an Spatio-Temporal Action Graph Network Module which outputs a video representing $1 \times d$ processed by an attention over frames and objects from the new and improved \ignore{$\ve'{_{i}^{t}}$} features using graph networks approach. (4) Last, the model outputs collision classification.}
\label{fig:system}
\end{center}
\end{figure*}


\textbf{Video Activity Classification}
%Lisa: changed
%As the models for activity classification enter the era of deep learning, the earliest activity classification model takes the spirit of bag of words by pooling over the per-frame features of the whole video sequence~\cite{karpathy2014large}. 
Early deep learning activity classification systems are in the spirit of bag of words models: per-frame features are pooled over an entire video sequence~\cite{karpathy2014large}.
Simply pooling the per-frame features will ignore temporal structure in the video.
Later work used a recurrent neural network, such as an LSTM, to temporally aggregate per-frame features\cite{donahue2015long,yue2015beyond}.
Another line of activity classifiers use 3D spatio-temporal filters to create hierarchical representations of the whole input video sequence~\cite{ji20133d,taylor2010convolutional,tran2015learning,varol2018long}. While spatio-temporal filters can benefit from large video datasets, they cannot be pretrained on images.
%are prohibited from image pretrain. 
Two-stream networks are proposed to leverage image pretraining in RGB as well as capturing fine low-level motion in another optical flow stream~\cite{simonyan2014two,feichtenhofer2016convolutional}.
I3D\cite{Carreira2017QuoVA} is designed to inflate 2D kernels to 3D to learn spatio-temporal feature extractors from video while leveraging image pretrain weights.
In all these aforementioned activity classifiers, whole frame video features are extracted without looking into the object details inside each frame. Our paper tries to investigate the spatio-temporal relationship of objects for activity classification.




\textbf{Objects for Activities}
Object interactions have been utilized for tackling various activity classifications, e.g. image activity classification, spatial-temporal activity detection, video activity classification. 
\cite{li2007and} classifies image events by modeling scene and object interactions.
In still images, \cite{yao2012recognizing} shows that objects and human poses can serve as mutual context and facilitate the recognition of each other in human-object interaction activities.
\cite{sun2018actor,girdhar2018video} capture the interactions of human actors, relevant objects and global scene features, and accumulate relation information for classifying localized action proposals in spatio-temporal activity detection task. 
In video classification, the traditional graphical models such as Hidden Markov model and Bayesian Network are combined with object context to classify hand actions~\cite{moore1999exploiting}, or used to incorporate semantic/functional and spatial context for action recognition~\cite{gupta2009observing}.
\cite{ryoo2007hierarchical,fathi2011understanding} model human-object interactions or object-hand interactions in probabilistic hierarchical way.
\cite{wu2007scalable} proposes an approach for activity recognition based on detecting and analyzing the temporal sequence of objects using dynamic Bayesian network.

Beside utilizing traditional graphical models in video activity classification, recently some works have investigated the effect of object relations in activity classification~\cite{Wang_videogcnECCV2018,baradel2018object,ma2017attend} using deep learning based graph models, and our paper follows this direction.

%and investigates the spatio-temporal relationship of objects for activity classification.
%\cite{moore1999exploiting} is the early work to exploit human motion and object context to perform action recognition and object classification. 
%Since most activity classifications tasks are related to human, a batch of papers modeling the interaction of human and objects for activity recognition emerged~\cite{ryoo2007hierarchical,gupta2009observing,yao2012recognizing}.
%Lisa: change
%Since many activity classes are related to humans, a variety of papers aim to model the interaction of human and objects for activity recognition
%exploits the consistent appearance of objects, hands, and actions from the egocentric view for activity recognition. 
%joint modeling of activities, actions, and objects leads to superior performance in comparison to the case where they are considered independently.


%We investigate spatio-temporal object interactions in the car-road scene for collision classification, and demonstrate the benefit of explicit modeling object relationships through space and time.





%models short temporal snapshots of videos by averaging the predictions from a single RGB frame and a stack of 10 externally computed optical flow frames, after passing them through two replicas of an ImageNet pre-trained ConvNet. 

% STAG figure
\begin{figure*}[t!]
    \begin{center}
        \includegraphics[width=\linewidth]{Figures/stag_arch_iccv.png}
    \caption{A schematic representation of the \textbf{Spatio-Temporal Action Graph Network} Module.
    (a) First, the features $\ve_{i}^{t}$ and $\ve_{i,j}^{t}$ are processed by a FC layer to a feature space of dimension $d$. (b) The node and edge features are processing using a H-NL block in the Message Passing Hierarchy to get an improved node features. (c) The Spatial Context Hierarchy pooling over the spatial dimension to get frame features. Given the frame features and the node features, the H-NL block outputs an improved frame features. (d) Then, the Temporal Context Hierarchy pooling over the temporal dimension to get a video feature, and the rest of process of H-NL block is the sames as the previous stage. The final output is an improved video feature to contain the entire scene information.}
    \label{fig:actions_graph}
    \end{center}
\end{figure*}






\textbf{Graph Models}
Traditional graph models include Hidden Markov Model~\cite{krogh2001predicting}, Bayesian Network~\cite{nielsen2009bayesian}, Conditional Random Field\cite{lafferty2001conditional}, etc.
Graph models have been applied on many computer vision applications, including scene graph for rich image representation in the image retrieval task~\cite{johnson2015image}, visual relational reasoning~\cite{battaglia2018relational,zambaldi2018relational,baradel2018object}, image generation~\cite{johnson2018image}, robotics~\cite{sanchez2018graph}, etc.
Defining the graph structure and the policy to pass message between nodes are two important aspects when using graph models.
Traditional graph structure can be either hand defined using prior knowledge or learn from data in a probabilistic way using heuristic methods like greedy search~\cite{tsamardinos2006max}. 
The junction tree inference algorithm~\cite{wainwright2008graphical} is a popular message passing algorithm in Bayesian graphical model.
Recently, deep learning based graph structure learning models for computer vision problems
have been proposed~\cite{yang2018graph,qi2018learning}.
\cite{yang2018graph} automatically constructs scene graph based on Faster R-CNN architecture.
The massage passing algorithm has been redefined as various graph convolution operations~\cite{herzig2018mapping,kipf2016semi} in deep graph models.
In this paper, we define the initial graph structure based on the union of boxes with the goal of utilizing the spatial layout information for video activity classification.
Additionally, we further refine the graph connection and learn a latent spatial-temporal graph connection using attention mechanism to pass information between neighbour nodes and aggregate context information.
% edge features
% message passing....
% latent connection
%we build an object graph model to improve performance on video activity classification tasks.

\textbf{Attention Mechanism}
Attention mechanism is essentially weighting the context features based on the similarities of current object and its contexts.
In early stage, attention mechanism has been successfully deployed for various natural language and computer vision tasks like machine translation~\cite{bahdanau2014neural}, visual question answering~\cite{xu2016ask}, image captioning~\cite{xu2015show}, video captioning~\cite{yao2015describing}, etc.
%attention is all you need
\cite{vaswani2017attention} gives the concept of ``self-attention" with the two interaction objects being the same object, and proposes the transformer model based solely on attention dispensing the recurrence network taken in previous attention based machine translation model~\cite{bahdanau2014neural}.
%Both convolutional and recurrent operations are building blocks that process one local neighborhood at a time.
%this paper, we present non-local operations as a generic family of building blocks for capturing long-range dependencies. 
\cite{wang2018non} inherits the ``self-attention" concept and defines the non-local operation by computing the response at a position as a weighted sum of the features at all positions for video classification. 
Later on, Wang, etc~\cite{Wang_videogcnECCV2018} propose to represent videos as space-time region graphs with object region proposals as nodes and perform reasoning on this graph representation via Graph Convolutional Networks.
Their graph convolutional operation is essentially equivalent to ``non-local operation"\cite{wang2018non} as well as the self-attention concept.
%These nodes are connected by two types of relations: (i) similarity relations capturing the long range dependencies between correlated objects and (ii) spatial-temporal relations capturing the interactions between nearby objects. 
\cite{wu2018long} modifies the non-local operation to aggregate temporal context for video classification and action detection.
We propose a hierarchical graph model for video classification and aggregate spatial-temporal context using attention.

%To understand the world, we humans constantly need to relate the present to the past, and put events in context.
%In this paper, we enable existing video models to do the same. 
%We propose a long-term feature bank—supportive information extracted over the entire span of a video—to augment state-of-the-art video models that otherwise would only view short clips of 2-5 seconds. 



\textbf{Autonomous Driving}
Neural network could mimic humans driving~\cite{pomerleau1989alvinn}. Recently, deep learning has been applied to learn self-driving policy~\cite{chen2015deepdriving,bojarski2016end}, and key objects such as lane markings and nearby vehicles are important for perceiving the scene in autonomous driving system~\cite{bojarski2017explaining}. Collision avoidance is an important goal for self-driving system~\cite{kahn2017uncertainty}, and it needs both sensor and vision data to make reliable prediction.
Collision vision data is difficult to collect in the real world since these are unexpected rare events.
\cite{kim2019crash} tackles the collision data scarcity by developing synthetic data using driving simulator. However there still exists domain gap between synthetic collision data and real collision data.
In this paper, we introduce a challenging collision dataset based on real-world dashcam data. 
At the same time, we propose a hierarchical graph model suitable for classifying rare events by modeling the key object interactions with limited training examples.

%like vehicles and pedestrians  in autonomous driving system .


%In (Kahn et al. 2017; Thorsson and Steinert 2016), the authors apply reinforcement learning to develop collision avoidance systems. 
%Despite of the huge success, these approaches cannot efficiently predict and handle dangerous scenarios, which are rarely observed during training. 
%Thus, our collision predic- tion algorithms can provide an additional level of safety to self-driving and collision avoidance systems.
%However, these approaches typically assume availability of expensive devices (such as radar, LIDAR, or communication chips) to measure or receive the states of nearby vehicles.
%To avoid the dependency on expensive hardwares, one may make use of low-cost cameras by developing a com- puter vision-based collision prediction systems. 
%In a few re- cent works, the authors propose the use of convolutional neural networks (CNNs) for building efficient CPS (Wang and Kato 2017; Suzuki, Aoki, and Kataoka 2017; Chan et al. 2017). 
%However, they could collect only a small amount of accident data due to data scarcity and difficulty of manual annotation. 



% Removed for now

% \huijuan{maybe remove the following parahraph about "object detection"}

% \textbf{Object Detection}
% Faster R-CNN~\cite{ren2015faster}, extends R-CNN~\cite{girshick2014rich} and Fast R-CNN~\cite{girshick2015fast} object detection approaches, incorporating region of interest (RoI) pooling and a region proposal network.
% More recent object detection models include SSD~\cite{liu2016ssd}, R-FCN~\cite{li2016r} and YOLO~\cite{redmon2016you} which achieve faster and better object detection.
% Mask R-CNN~\cite{he2017mask} extends Faster R-CNN by adding one extra branch for predicting object masks in parallel with original bounding box predictions.
% It efficiently detects objects in an image while simultaneously generating a high-quality instance segmentation mask.
% In this paper we take the high quality proposals to build the spatial-temporal graph over them for activity classification.
% Object detection proposals serve as a foundation for several computer vision tasks like visual grounding~\cite{hu2016natural}, robot learning~\cite{devin2018deep} etc.
% Here we try to leverage the object proposals for activity classification task.



==> Sections/old_03_model.tex <==


\section{Spatio-Temporal Action Graph}
\label{sec:model}


% disentangle
%In what follows we describe our model for object-aware recognition using a Spatio-Temporal Action Graph Network (STAG). 
In this section we describe our proposed Spatio-Temporal Action Graph Network (STAG) with object interaction modeling to improve video recognition. 
Our main challenge was doing a dimension reduction of the 3-D input to 1-D compact vector, in a way that mixed information from both the spatial and temporal space.
While the global pooling of convolutional filter output might ignore some crucial features for discriminating actions, object interaction modeling can compensate and capture important clue inside the video clip.
\roeih{It's unclear need to rephrase it}
But general object interactions with attention for the whole video might still miss important things happening inside each frame.
We disentangle the object spatial interaction and temporal interaction into two hierarchies, and do attention first within each frame and then temporally between frames.
By the structural attention hierarchies disentangling spatial and temporal interactions, we expect STAG can attend to important factors in each frame for better action classification.



%The key insight of the Spatio-Temporal Action Graph module is that is that actions are characterized by the way different objects interact in the image across space and time. 
The overall Object-Aware Action Recognition architecture is shown in \figref{fig:system}.
%
%We next describe each of the components in more detail. 
%In what follows we use the following constants: 
Given $T$ input frames in the video sequence to be classified, Our model fuses two different kinds of video encoding with compensating effects for final classification, namely the global pooling branch over direct 3D convolutional feature encoding and the object interaction branch which models the hierarchical spatial and temporal interactions using our proposed STAG module.

%$N$ is the maximum number of objects (i.e., bounding boxes) per frame, and $d$  is the dimensionality of feature vector for each bounding box (as calculated by the Mask R-CNN).  We also use $[T]$ to denote the set $\{1,\ldots,T\}$ and $[B]$ to denote the set $\{1,\ldots,N\}$.
%\textbf{Object-aware Activity Recognition architecture}. The input consists of a sequence of 20 frames. (1) A backbone of ResNet50 and RPN produces a set of bounding boxes proposals for each frame. (2) A \textit{RoiAlign Single} layer extracts $\ve_{i}^{t}$ features from the backbone using the boxes. In parallel, every pair of box proposals is used for computing a union box, and  pairwise features $\ve_{i,j}^{t}$ extracted similar to the $\ve_{i}^{t}$ features. (3) The $\ve_{i}^{t}$ and $\ve_{i,j}^{t}$ are used as inputs to an Spatio-Temporal Action Graph Network Module which outputs a video representing $1 \times d$ processed by an attention over frames and objects from the new and improved \ignore{$\ve'{_{i}^{t}}$} features using graph networks approach. (4) Last, the model combines object interaction and global pooling video features to predict collision.
%To capture these, our model is constructed as follows. 

A detailed diagram of STAG Module is shown in \figref{fig:actions_graph}.
Our STAG module is built on top of the bounding boxes detected on each frame. Notably, Beside directly using the Region of Interest (RoI) features of the bounding boxes, we also use RoI features from the union of bounding boxes to capture the pairwise spatial appearance feature.
The object interactions inside STAG model are broken into two hierarchies which are spatially and temporally disentangled, namely the spatial context hierarchy and temporal context hierarchy.
In the spatial hierarchy, the object interactions are limited within each frame to fully explore the spatial interaction of objects falling in the same frame.
On top of the spatial hierarchy, we further pool over the structural spatial representation to get one per-frame feature representation with strong spatial interaction encoding.
Next in the temporal hierarchy, information is passed across the aforementioned per-frame features with temporal attention. 
And a final temporal pooling generates the representation for the entire input video sequence, 
which is combined with the global pooling features for classifying the action.  
By purposely disentangling the spatial-temporal interactions into two hierarchies, we get rich spatial-temporal information with focus on video-based key objects for better action recognition.
We next describe the components inside the STAG model in more details.


%Those, design choices in the above architectures are specifically targeted at modeling spatio-temporal patterns, whereby information is gradually aggregated along both these axes.
%box
%First, a detector module is applied to the image to extract bounding boxes of objects of interest (see Section \ref{sec:model:detector}). This results in a set of vector representations for the bounding boxes, and pairs of bounding boxes. This is done for each time-frame in the sequence. 
%spatial
%Next, these representations are re-processed via a graph network, resulting in a new representation per box, where now each such representation has incorporated information from all other boxes. Therefore, the new representation can take context into account. Again, this is done per time-frame. Additionally, at each time frame, a per-frame representation is calculated.
%temporal
%Finally, information is aggregated across frames, by using a variant of an attention module. This results in a representation of the entire sequence, which is then used for classifying the action. Those, design choices in the above architectures are specifically targeted at modeling spatio-temporal patterns, whereby information is gradually aggregated along both these axes.

% merge to the next sections...

% % Hierarchy Non Local Block figure
% \begin{figure}[t!]
%     \begin{center}
%         \includegraphics[width=0.8\linewidth]{Figures/hier_non_local3_iccv.jpg}
%         % Figures/modified_non_local2_iccv.jpg
%     \caption{Hierarchical Non-Local (H-NL) block. The inputs $x_{1}$ and $x_{2}$ have $\mathbb{R}^{N}$ and $\mathbb{R}^{N+1}$ dimensions correspondingly, and the output dimension $y$ is the same as $x_{1}$. Here we used $N=3$, but it can be generalized for any $N$. The output $y$ is an improved $x_{1}$ feature. \roeih{Need to explain it?}}
%     \label{fig:comparing_blocks}
%     \end{center}
% \end{figure}


% Mask RCNN
%\subsection{Detector}
\subsection{Graph Generator}
\label{sec:model:detector}
Before applying the two disentangled spatial and temporal context aggregations, we need to construct one initial graph representation encoding objects and their relations. As a first step, we detect region proposal boxes and extract corresponding box features through an RoIAlign layer by object detection Faster R-CNN~\cite{faster_rcnn}. Instead of only using object features with their bounding boxes, we believe that the spatial relation of each pair of bounding box should be important and encoded into the initial graph representation for subsequent spatial and temporal context aggregation. Specifically, for each pair of boxes, we consider its union (see \figref{fig:system}) and use an RoIAlign layer to extract the union box features as initial edge features with the union boxes capturing the spatial appearance of each pair of objects.

%\textit{RoIAlign Single} and \textit{RoIAlign Pairwise} layers that removed the harsh quantization and properly aligning the extracted features with the input. Given an image, the convolutional network produce a feature map, from which the RPN generates a list of candidate objects proposal. The \textit{RoIAlign} layer gets the feature map and list of objects proposals as an input and predict category label for each object feature by applying two FCNs.


We now give the notation definitions. In what follows we use the following constants: $N$ is the maximum number of objects (i.e., bounding boxes) per frame, and $d$  is the feature dimensionality.  We also use $[T]$ to denote the set of input frames $\{1,\ldots,T\}$ and $[B]$ to denote the set of bounding boxes in each frame $\{1,\ldots,N\}$.
The detection stage therefore results in two sets of tensors shown in \figref{fig:actions_graph} (a): 
\begin{itemize}
    \item Single-object features: For each time step $t\in[T]$ and box $i\in[B]$ we have a 
    feature vector $\ve_{i}^t\in\reals^d$ for the corresponding box. The feature contains the output of the RoIAlign layer.% and the bounding box coordinates.
    \item Object-pair features: For each time step $t\in[T]$ and box-pair $i\in[B],j\in[B]$ we have a feature vector $\ve_{i,j}^t\in\reals^d$ for the corresponding pair of boxes. The feature contains the output of the RoIAlign layer. %and the coordinates of the union bounding-box.
\end{itemize}


Thus overall, we have a tensor of size $T\times N \times d$ for single object features, and a tensor of size $T\times N\times N \times d$ for object-pair features. 
Next in \figref{fig:actions_graph} (b), we use these single object features and object-pair features to construct a graph feature representation. Firstly, the initial node features $\ve_{i}^{t}$ and union box edge features $\ve_{i,j}^{t}$ are embedded into feature space with dimension $d$. Then we concatenate each edge features with the two connected node features and further embed it into dimension $d$ to form one aggregated representation with objects and their interactions. 



% Action Graph Networks
\subsection{STAG Module}
\label{sec:model:actions_net}
After getting the aggregate features $T\times N\times N \times d$ with rich spatial appearance of object interactions from Fig.~\ref{fig:actions_graph} (b), we will allow the objects to exchange information with each other and aggregate context from neighbourhoods to further form a video descriptor for action classification.
We build a structural model with the spatial hierarchy (see Fig.~\ref{fig:actions_graph} (c)) and temporal hierarchy (see Fig.~\ref{fig:actions_graph} (d)) in sequence.
The message passing in the spatial hierarchy is constrained to be the objects features within each frames, while the one at the temporal hierarchy is constrained to the sequence of whole frame encoding.
Inspired by recent graph model~\cite{mapping_to_imgs}, we take attention mechanism to realize the message passing between objects, more specifically, we take the self-attention based Non-local operations proposed in~\cite{wang2018non}.
%In order to model the interaction between multiple objects in the same frame, we use a graph network that integrates information across all boxes and pairs of boxes in a single frame. 
%old H1
%At the first, the features of $\ve_{i,j}^t$ are processed element-wise by $\alpha$. 
%Then, a reduction step a tensor of size $T\times N\times N\times d$ is reduced to $T\times N\times d$ by having each box ``attend'' to all the other boxes, thereby integrating information from across the frame. 
%old H2
%After that, those features, are processed by $\beta$, and in the next reduction phase, $T\times N\times d$ is transformed to $T\times d$  via a soft-attention over boxes per time frame. 
%This results in a feature vector describing each complete frame. 
%old H2
%At this point, we reprocess the single box features $\zz_{i}^t$ using the complete frame features by $\gamma$ to get an improved features $\ve'{_{i}^{t}}$. 
%To obtain a representation for the whole sequence we reduce over $T\times N$ resulting in a vector $\reals^d$ for the entire sequence. 
%Finally, we apply a multi-layer neural network to this vector, with a softmax classifier. 
%As we described later in \secref{sec:exper:details}, $\alpha$, $\beta$ and $\gamma$ are functions mapping features from one dimension to another.
%The way we implement this idea in the network architecture is by using soft attention on the objects (see model description above), in order to reduce the object axis, allowing the network to concentrate on specific objects. 
Before we introduce the two hierarchies in details, Let us first recap the Non-local operation in~\cite{wang2018non}.

\textbf{Non-local Operation.}
Non-local operations \cite{wang2018non} are an efficient, simple and generic component for capturing long range dependencies. We define the generic operation for our edge-graph as the following:

\begin{equation}
\label{eq:edges_nonlocal}
% \vect{y}_i = \frac{1}{\mathcal{C(\ve)}} \sum_{\forall j}f(\ve_i, \ve_j)g(\ve_j)
\vect{y}_{i,j} = \frac{1}{\mathcal{C(\ve)}} \sum_{\forall k, l}f(\ve_{i, j}, \ve_{k, l})g(\ve_{k, l})
\end{equation}

while $(i,j)$ is the index of a given edge box descriptor whose response to all other $(k, l)$ edges descriptors per frame. $\ve$ is the input signal and $\vect{y}$ is the output of signal of the same size as $\ve$. A pairwise function $f$ represents the interactions between edges over time between each edge $(i,j)$ to all other edges $(k, l)$. The unary function $g$ computes a representation of the input signal of the edge feature. 

In addition, we also use the generic operation for over the temporal dimension the same as the original non-local operation as in \cite{wang2018non}:
\roeih{The second formula is not clear. You are using the same notations but it can't be the same functions.}
\begin{equation}
\label{eq:temp_nonlocal}
\vect{y}_i = \frac{1}{\mathcal{C(\ve)}} \sum_{\forall j}f(\ve_i, \ve_j)g(\ve_j)
\end{equation}

\textbf{Spatial Context Hierarchy.}
The Spatial Context Hierarchy (\figref{fig:actions_graph} (c)) uses the Non-Local block to obtain improved edge features and then pools over the spatial dimension to get frame features. First, given the edge features $\ve_{i, j}$ 
the Non-local block, as mentioned in \eqref{eq:edges_nonlocal}, has been modeling the \roeih{?? missing words} to get a better edges features. Then, we use a spatial average pooling operator to get the frame features of ~$T \times d$ dimensions.   



\textbf{Temporal Context Hierarchy.}
Then, the Temporal Context Hierarchy (\figref{fig:actions_graph} (d)) uses a Non-Local block (see \eqref{eq:temp_nonlocal}) to get an improved frame features and pooling over the temporal dimension. The final output is an improved video feature containing the entire scene information and video dynamics of ~$1 \times d$ dimensions.



%The motion of the objects is a critical key in order to correctly recognize the action in a video clip. 
%Since the order of the detected objects will typically vary between different frames (as it just corresponds to the order in which the RPN ranks these), there is a need to align the objects in order to mix the objects information across the temporal dimension. 
%In cases where there is a need to recognize activity of one main object (such as car collisions), the network architecture can exploit this property and concentrate on one object at each frame. 

%The way we implement this idea in the network architecture is by using soft attention on the objects (see model description above), in order to reduce the object axis, allowing the network to concentrate on specific objects. 
%Thus, instead of explicitly modeling all object interactions between frames (which requires a fixed object ordering across all frames), we first aggregate object relationships, then model temporal relationships. 
%After the dimensions reduction, we left with one feature vector per frame. We then combine all the frames together, reduced the temporal dimension and predict the action.


% It proceeds in the following steps:
% \begin{itemize}
%     \item Pre-process pairwise - Apply a network $F_1$ to each pairwise feature $\ve_{i,j}^t$. Denote the output by $\uu_{i,j}^t.$
%     \item Summarize pairwise boxes - For each box $i$, take a weighted sum over $\uu_{i,j}^t$, where the weights are determined by an attention mask, whose weights are calculated from $\zz_{i}^t$ \amirg{Is this correct}. This results in a tensor of size $T\times N\times d$, which has features for all boxes in all frames. This new representation incorporates information from all boxes.\amirg{Where does $\zz_{i}$ come into this? Just attention?} 
%     \item Post-process pairwise - Apply a network $F_2$ to each feature vector in the above $T\times N\times d$ tensor. This results in a $T\times N\times d$ tensor.
%     \item 
% \end{itemize}


% We now construct a graph, using Action Graph Network Module, which contains $N$ nodes corresponding to $N$ object proposals aggregated over $T$ frames. Action Graph Network Module is a graph network based on \cite{mapping_to_imgs} for a deep structured prediction. Given an input of 
% $\ve_{i,j}^{t}$, the architecture "collects" information from all different edges of the graph, such it first aggregate all the features around a given node. Then, there is an attention over the nodes to get a scene representation per frame. Combining the node features $\ve_{i}^{t}$ with those scene representation per frame, outputs an improved node (object)  features $\ve'{_{i}^{t}}$ which enriched by the all frame scene  (Fig.~\ref{fig:actions_graph}). Last, an attention mechanism over the frames and object is been performed to extract the entire video sequence representation. 

%Finally, features from the video sequence representation are concatenated with the image features taken from ResNet last layer after global average pooling over $T \times H \times W$ is, and fully connected feed forward network applied to classify each of video to either “collisions” or “no collision”. 


%The motion of the objects is a critical key in order to correctly recognize the action in a video clip. Since the order of the detected objects will typically vary between different frames (as it just corresponds to the order in which the RPN ranks these), there is a need to align the objects in order to mix the objects information across the temporal dimension. In cases where there is a need to recognize activity of one main object (such as car collisions), the network architecture can exploit this property and concentrate on one object at each frame. 

%The way we implement this idea in the network architecture is by using soft attention on the objects (see model description above), in order to reduce the object axis, allowing the network to concentrate on specific objects. Thus, instead of explicitly modeling all object interactions between frames (which requires a fixed object ordering across all frames), we first aggregate object relationships, then model temporal relationships. After the dimensions reduction, we left with one feature vector per frame. We then combine all the frames together, reduced the temporal dimension and predict the action. 




% % Attention figure
% \begin{figure}[t!]
%     \begin{center}
%         \includegraphics[width=\linewidth]{Figures/attention_fig2.jpg}
%     \caption{Attention mechanism for object alignment: in the above example we can see in each frame the object with the highest attention score. This turns out to be, in most of the frames, the truck involved in the collision, even though the RPN outputs the corresponding box at a different index in each frame. Therefore, the attention mechanism effectively aligns the car across frames.}
%     \label{fig:attention_graph}
%     \end{center}
% \end{figure}



%In order to model the interaction between multiple objects in the same frame, we use a graph network that integrates information across all boxes and pairs of boxes in a single frame. The network, inspired by the architecture in \cite{mapping_to_imgs}, is shown in Fig.~\ref{fig:actions_graph}. It progressively aggregates over information to eventually obtain a vector in $\reals^d$ describing the whole sequence. At the first, the features of $\ve_{i,j}^t$ are processed element-wise by $\alpha$. Then, a reduction step a tensor of size $T\times N\times N\times d$ is reduced to $T\times N\times d$ by having each box ``attend'' to all the other boxes, thereby integrating information from across the frame. After that, those features, are processed by $\beta$, and in the next reduction phase, $T\times N\times d$ is transformed to $T\times d$  via a soft-attention over boxes per time frame. This results in a feature vector describing each complete frame. At this point, we reprocess the single box features $\zz_{i}^t$ using the complete frame features by $\gamma$ to get an improved features $\ve'{_{i}^{t}}$. To obtain a representation for the whole sequence we reduce over $T\times N$ resulting in a vector $\reals^d$ for the entire sequence. Finally, we apply a multi-layer neural network to this vector, with a softmax classifier. As we described later in \secref{sec:exper:details}, $\alpha$, $\beta$ and $\gamma$ are functions mapping features from one dimension to another.

